Modelling Bushfire Evacuation Behaviours

Bushfires pose a significant threat to Australia's regional areas. To minimise risk and increase resilience, communities need robust evacuation strategies that account for people's likely behaviour both before and during a bushfire. Agent-based modelling (ABM) offers a practical way to simulate a range of bushfire evacuation scenarios. However, the ABM should reflect the diversity of possible human responses in a given community. The Belief-Desire-Intention (BDI) cognitive model captures behaviour in a compact representation that is understandable by domain experts. Within a BDI-ABM simulation, individual BDI agents can be assigned profiles that determine their likely behaviour. Over a population of agents their collective behaviour will characterise the community response. These profiles are drawn from existing human behaviour research and consultation with emergency services personnel and capture the expected behaviours of identified groups in the population, both prior to and during an evacuation. A realistic representation of each community can then be formed, and evacuation scenarios within the simulation can be used to explore the possible impact of population structure on outcomes. It is hoped that this will give an improved understanding of the risks associated with evacuation, and lead to tailored evacuation plans for each community to help them prepare for and respond to bushfire.

==> chapter-theory/subsec-attributes.tex <==
\subsection{Attributes}

The above algorithm creates a plan that is ready for MATSim to use on a regular day, but it will not contain any of the information required to describe how the agents will act in a bushfire.
To do this, we append attributes to each agent that describe things like how much risk they are willing to tolerate before evacuating, where they will go if they do choose to leave, and what responsibilities they will have before leaving.
Once these have been determined, the agent will be ready to react to a bushfire threat in a simulation environment that executes a rich cognitive architecture alongside the traffic simulation.
Below we will describe how the behavioural model is designed, and how the attributes are assigned to agents from an additional set of inputs.
\subsubsection{Threshold Model}
Most major research regarding bushfire behaviour concerns if and when people will evacuate in the face of threat, and this decision is central to the behavioural model.
An important factor to consider was the amount of opportunities an agent would have to to decide to leave, and how to capture this build up of information and pressure without having all agents eventually deciding to leave.
This means that a probabilistic approach to the decision, where an agent has a certain likelihood of leaving after receiving a given percept, is difficult to control and unlikely to give a realistic representation of a person's actions; if each agent receives a percept enough times it will eventually cause them to leave, even if individually the percept carries a low probability of triggering an evacuation.
In trying to capture the diversity of reactions in a community, it is important to not let the response be skewed by this cumulative effect.
\\

For this reason, we employ a threshold-based model, where each agent has an intrinsic value which determines how they respond to a threat, and allows for the agent to remember the previous percepts they have been exposed to when making their decision.
Relevant percepts are broken up into two categories.
\textsc{Environmental} alerts pertain to information gleaned directly from the surroundings.
They will include embers, smoke, flames, the movement of neighbouring agents, and the actions of emergency services in the vicinity.
\textsc{Transmitted} alerts include those that are issued by the emergency authorities before and during a bushfire emergency and other messages received via the media or other communications networks.
Let $E$ and $T$ denote the sets of all alerts $e$ and $\tau$ for each category.
Both sets are totally ordered
\begin{align*}
  e_1\leq e_2 \leq e_3 \leq e_4\leq...\leq e_n ,\\
  \tau_1\leq \tau_2 \leq \tau_3 \leq \tau_4\leq...\leq \tau_m
\end{align*}


i.e. we denote the severity of each percept relative to the others in its category.
Whenever an agent receives a percept, it will update their `barometer' for the corresponding alert type.
The two categories differ here in that the \textsc{Environmental} barometer will only update if the new alert is of greater severity than the previous barometer alert, whereas the \textsc{Transmitted} barometer will also allow updates to a reduced level of threat.
This reflects the nature of the different alert types; if you see smoke, it doesn't reduce the threat of the flames you had seen earlier, but if you receive a less severe warning from an authority it is likely to decrease the concern caused by an earlier warning message.
We now have a way of capturing the different types of threat percepts that might trigger an evacuation, defined a method of updating the severity level of the threat, and separated the percepts into groups that broadly maintain a distinction between primary and secondary information.
\\

We now must combine these two barometers into one value that reflects a person's overall threat level. If we consider
$$
E\times T=\{ \{0,0\},\{e_1,0\},\{0,t_1\},\{e_1,t_1\},...,\{e_n,t_m\}\}
$$

representing the set of all combinations of alerts that an agent may have registered as their barometer at some time (with $0$ representing no threat of that type being received).
There is naturally a partial ordering on the ordered pairs with each fixed value of $e_n$ or $t_m$ (stemming from the ordering in the other category set).
However, there is no defined order of, say, $\{e_1,t_3\}$ and $\{e_2,t_2\}$.
We therefore need to define a mapping

$$r: E\times T \longrightarrow (0,1)$$

which maintains all partial orders and also defines the correct order between each undefined element pairs. Note that the value set that $r$ maps to is arbitrary, and serves only to quantify the ordering into a ranking score.
We may then have the case that, say, $r(\{e_1,t_3\})=r(\{e_2,t_2\})$ i.e. an agent can arrive at a ranking score through various different combinations of alerts. The ranking $r$ of the current barometer levels is then compared against the agent's intrinsic tolerance score \texttt{tol}, and if $r>\tt tol$ then the agent will change their daily plan.



\subsubsection{BDI Attributes}

\subsubsection{Assigning Attributes}


==> macros.tex <==
%!TEX root = ../thesis.tex

\newcommand{\mathname}[1]{\operatorname{\textit{#1}}}
\newcommand{\superscript}[1]{\ensuremath{^{\textrm{#1}}}}
\newcommand{\subscript}[1]{\ensuremath{_{\textrm{#1}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PERSONAL LaTex MACROS 
% Courtesy Sebastian Sardina, RMIT Melbourne.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Font modes & definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% conditional math environment
% \gdef\Math#1{\ifmmode #1 \else \mbox{$#1$}\fi}
\newcommand{\Math}[1]{\ensuremath{#1}}

\newcommand{\modesf}[1]{{\Math{\mathsf{#1}}}}
\newcommand{\modecal}[1]{{\Math{\mathcal{#1}}}}
\newcommand{\modeit}[1]{{\Math{\mathit{#1}}}}


\newcommand{\textmath}[1]{{\mbox{\textit{#1}}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Proper names
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\propername}[1]{\mbox{\small\textsf{#1}}}
\newcommand{\AgentO}{\propername{AGENT-0}}
\newcommand{\AgentSpeak}{\propername{AgentSpeak(L)}}
\newcommand{\AgentSpeakF}{\propername{AgentSpeak(F)}}
\newcommand{\ASHOP}{\propername{A-SHOP}}
\newcommand{\CANMINUS}{\propername{\CAN$^{\A}$}}
\newcommand{\CANMINUST}{\propernametiny{Can$^{\cal C}$}}
\newcommand{\CAN}{\propername{CAN}}
\newcommand{\CANT}{\propernametiny{Can}}
\newcommand{\CANPLAN}{\propername{CANPlan}}
\newcommand{\CANPLANT}{\propernametiny{CanPlan}}
\newcommand{\CANPLANII}{\propername{CanPlan2}}
\newcommand{\CANPLANOR}{\propername{Can(Plan)}}
\newcommand{\CANGOAL}{\propername{CanGoal}}
\newcommand{\ConGolog}{\propername{ConGolog}}
\newcommand{\CLAIM}{\propername{CLAIM}}
\newcommand{\dMARS}{\propername{dMARS}}
\newcommand{\DAPL}{\propername{2APL}}
\newcommand{\GOAL}{\propername{GOAL}}
\newcommand{\GOALBDI}{\propername{GOAL}}
\newcommand{\Golog}{\propername{Golog}}
\newcommand{\GORITE}{\propername{GORITE}}
\newcommand{\IndiGolog}{\propername{IndiGolog}}
\newcommand{\JACK}{\propername{JACK}}
\newcommand{\JACKTM}{\propername{Jack\texttrademark}}
\newcommand{\JADEX}{\propername{JADEX}}
\newcommand{\JAM}{\propername{JAM}}
\newcommand{\JASON}{\propername{Jason}}
\newcommand{\JSHOP}{\propername{JSHOP}}
\newcommand{\JSHOPII}{\propername{JSHOP2}}
\newcommand{\PDT}{\propername{PDT}}
\newcommand{\PLACA}{\propername{PLACA}}
\newcommand{\Prometheus}{\propername{Prometheus}}
\newcommand{\PRS}{\propername{PRS}}
\newcommand{\RAP}{\propername{Rap}}
\newcommand{\SHOP}{\propername{SHOP}}
\newcommand{\SHOPII}{\propername{SHOP2}}
\newcommand{\SPARK}{\propername{SPARK}}
\newcommand{\TAPL}{\propername{3APL}}
\newcommand{\weka}{\propername{weka}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Calligraphic letters 
% -- Taken from Giuseppe De Giacomo 2006
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\A}{\modecal{A}} \newcommand{\B}{\modecal{B}}
\newcommand{\C}{\modecal{C}} \newcommand{\D}{\modecal{D}}
\newcommand{\E}{\modecal{E}} \newcommand{\F}{\modecal{F}}
\newcommand{\G}{\modecal{G}} \renewcommand{\H}{\modecal{H}}
\newcommand{\I}{\modecal{I}} \newcommand{\J}{\modecal{J}}
\newcommand{\K}{\modecal{K}} \renewcommand{\L}{\modecal{L}}
\newcommand{\M}{\modecal{M}} \newcommand{\N}{\modecal{N}}
\renewcommand{\O}{\modecal{O}} \renewcommand{\P}{\modecal{P}}
\renewcommand{\S}{\modecal{S}} \newcommand{\T}{\modecal{T}}
\newcommand{\U}{\modecal{U}} \newcommand{\V}{\modecal{V}}
\newcommand{\W}{\modecal{W}} \newcommand{\X}{\modecal{X}}
\newcommand{\Y}{\modecal{Y}} \newcommand{\Z}{\modecal{Z}}
\newcommand{\R}{\modecal{R}} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Margin notes for comments  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\marginparwidth}{0.1in}
\let\oldmarginpar\marginpar
\renewcommand\marginpar[1]{\-\oldmarginpar[\raggedleft\footnotesize #1]%
{\raggedright\footnotesize #1}}

\setlength{\marginparwidth}{0.5in}
\newcommand{\notem}[1]{\marginpar{\scriptsize  \textbf{#1}}}
\newcommand{\notems}[1]{\notem{S: #1}}
\newcommand{\noteml}[1]{\notem{L: #1}}
\newcommand{\notemd}[1]{\notem{D: #1}}

\newcommand{\ncheck}{\notem{CHECK!}}
\newcommand{\GGG}{\notem{GGG}}
\newcommand{\SSS}{\notem{SSS}}
\newcommand{\LIN}{\notem{LP}}
\newcommand{\YVES}{\notem{YL}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PhD boxed notes for the committee in Toronto 
% -- Taken from Ron Petrick 2004
% -- Modified
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{color}
\newcounter{countphdnote}
%\newcommand{\phdnote}[1]{\textbf{#1}}
\newcommand{\phdnote}[1]{
%\vskip 0.25in
\noindent
%\begin{center}
%\begin{tabular}{c}
		\fbox{
%		\fcolorbox{black}{white}{
%			\begin{minipage}{0.96\textwidth}
			#1\addtocounter{countphdnote}{1}%
%			\end{minipage}
			}
		\fcolorbox{black}{black}{\textcolor
		{white}{\textbf{\ Note \thecountphdnote\ }}}
%\end{tabular}
%\end{center}
%\vskip 0.25in
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tighter lists 
% -- Taken from Lin Padgham 2007
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcounter{bean}

\newenvironment{tightenumerate}{
                \begin{list}{
                  {\mbox {
                      \arabic{bean}.\/}}}{\usecounter{bean}
                      \setlength{\itemsep}{-1pt}\setlength{\topsep}{0pt}}}{
                \end{list}}

\newenvironment{tightitemize}{
                \begin{list}{$\bullet$}{
                    \setlength{\itemsep}{-1pt}}{\setlength{\topsep}{0pt}}}{
                \end{list}}
%\setlength{\itemsep}{0pt}}{\setlength{\topsep}{0pt}}}{

\renewenvironment{tightenumerate}{\begin{enumerate}}{\end{enumerate}}
\renewenvironment{tightitemize}{\begin{itemize}}{\end{itemize}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General useful macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Produces citations as follows: Author (Year)
\newcommand{\citeby}[1]{\citeauthor{#1} (\citeyear{#1})}

% Mark pages (pp. xxx)
\newcommand{\page}{pp.}

% Marker text
\newcommand{\marker}[1]{\textbf{******* \today: #1 *******}}

% Good underline --- Ttaken from Hector Levesque 2003
%	underline with space between text and line
\newcommand{\under}[1]{\mbox{\underline{\it\smash{#1}\vphantom{\lower.05ex\hbox{
x}}}}}

% \newcommand{\defterm}[1]{\under{\textit{#1}}}
\newcommand{\defterm}[1]{\textit{#1}}

% Comments -- just ignore everything: same as \comment{} in comment package
\newcommand{\commentarea}[1]{}

% Finish a page compactly (remove trailing space)
\newcommand{\finishpage}{ \newpage{ \pagestyle{empty} } }

% Separation for itemizations
\newcommand{\separation}[1]{\addtolength{\itemsep}{#1}}


% Italic text
\newcommand{\ii}[1]{\textit{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Thesis macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\subgoal}{sub-goal}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% EOF: macros-sebastian.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

